MITFAS: Mutual Information based Temporal Feature Alignment and Sampling for Aerial Video Action Recognition

We present a novel approach for action recognition in UAV videos. Our formulation is designed to handle occlusion and viewpoint changes caused by the movement of a UAV. We use the concept of mutual information to compute and align the regions corresponding to human action or motion in the temporal domain. This enables our recognition model to learn from the key features associated with the motion. We also propose a novel frame sampling method that uses joint mutual information to acquire the most informative frame sequence in UAV videos. We have integrated our approach with X3D and evaluated the performance on multiple datasets. In practice, we achieve 18.9% improvement in Top-1 accuracy over current state-of-the-art methods on UAV-Human(Li et al., 2021), 7.3% improvement on Drone-Action(Perera et al., 2019), and 7.16% improvement on NEC Drones(Choi et al., 2020).

==> figs/mitfas_rebu.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/mitfas_rebuttal.pdf}
    \caption{ More examples of the UAV data
    }
    \label{fig:uav}
\end{figure}

==> tables/Ablation_regionsize.tex <==
\begin{table}
% \footnotesize
\centering
% \begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c c c}
\toprule
Slipping Window Size & Frames & Top-1   \\
\midrule
0.15 &  $16$ &  $x$ \\
0.25 &  $16$ &  $x$ \\
0.5 &  $16$ &  $x$ \\
0.75 &  $16$ &  $x$ \\
\bottomrule
\end{tabular}
}
\caption{Results when human actor occupies different percentage of the frame}
\vspace{-5pt}
\label{tab:region}
% \end{center}
\end{table}

==> tables/Ablation_stride.tex <==
\begin{table}
% \footnotesize
\centering
% \begin{center}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c c c}
\toprule
Slipping Strides & Frames & Top-1   \\
\midrule
5 &  $16$ &  $52.7$ \\
10 &  $16$ &  $53.0$ \\
15 &  $16$ &  $52.8$ \\
20 &  $16$ &  $51.1$ \\
\bottomrule
\end{tabular}
}
\caption{Results when using different strides to calculate mutual information}

\label{tab:ablation_stride}
% \end{center}
\end{table}

==> tables/Ablation_study_shorter.tex <==
\begin{table}
% \footnotesize
\centering
% \begin{center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c | c c }
\toprule
Histogram Bin number & Top-1 & Reference image Size & Top-1 \\
\midrule
32 & $52.3$  & 1.10 $\times$ &  $53.4$  \\
64 & $52.7$  & 1.25 $\times$ &  $54.0$  \\
128 & $54.3$ & 1.5 $\times$  &  $53.7$  \\
256 & $52.7$ & 1.75 $\times$ &  $52.5$  \\
\bottomrule
\end{tabular}
}
\vspace{-7pt}
\caption{Ablation studies on UAV-Human subset in terms of using different bin numbers to calculate mutual information and reference image size (times of the standard size). The best performance is achieved while using 128 histogram bins and reference image size at 1.25$\times$.}
\vspace{-5pt}
\label{tab:ablation_s}
% \end{center}
\end{table}




==> tables/UAVHUMAN.tex <==
\begin{table}
%\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
Method & Backbone & Frames & Input Size & Init. & Top-1   \\
\midrule 
% X3D-S \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $21.5$ \\
X3D-M \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $27.0$ \\
X3D-L \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & None & $27.6$ \\
FAR \cite{divya2022far} & X3D-M & $16$ & $224\times 224$ & None & $27.6$ \\
FAR \cite{divya2022far} & X3D-M & $8$ & $540\times 540$ & None & $28.8$ \\
%AZTR & X3D-M & $16$ & $224\times 224$ & None & $39.2$ \\
\textbf{Ours (MITFAS)} & X3D-M & $16$ & $224\times 224$ & None & \textbf{40.2} \\
\midrule 
I3D \cite{carreira2017quo}& ResNet-101 & $8$ & $540\times960$ & Kinetics & $21.1$ \\
MViT  \cite{mvit}& - & $16$ & $224\times224$ & Kinetics & $24.3$ \\
X3D-M  \cite{feichtenhofer2020x3d}& - & $16$ & $224\times224$ & Kinetics & $30.6$ \\
FNet \cite{lee2021fnet} & I3D & $8$ & $540\times960$ & Kinetics & $24.39$ \\
FAR \cite{divya2022far} & I3D & $8$ & $540\times960$ & Kinetics & $29.2$ \\
FAR \cite{divya2022far} & X3D-M & $16$ & $224 \times 224$ & Kinetics & $31.9$ \\
FAR \cite{divya2022far} & X3D-M & $8$ & $620\times620$ & Kinetics & $39.1$ \\
%Diff-FAR \cite{kothandaraman2022fourier} & X3D-M & $8$ & $540\times540$ & Kinetics & $41.9$ \\
%Diff-FAR \cite{Kothandaraman2022DifferentiableFD} & X3D-M & $16$ & $540\times960$ & Kinetics & $40.8$ \\
%AZTR & X3D-M & $16$ & $224\times 224$ & Kinetics & $47.4$ \\
\textbf{Ours (MITFAS)} & X3D-M & $16$ & $224\times 224$ & Kinetics & \textbf{49.1} \\
\bottomrule 
\end{tabular}
}
\vspace{-7pt}
\caption{Benchmarking UAV Human and comparisons with prior arts. Our approach achieves a $13.2\%$ improvement over the baseline and $11.4\%$ over the current state-of-the-art when training from scratch. For initialization with Kinetics pretrained weights, MITFAS improves the top-1 accuracy over baseline by $18.5\%$ and over prior methods by at least $10.0\%$. More results using different input frame resolutions are provided in the supplementary materials.}
\vspace{-5pt}
\label{tab:uavhuman_sota}
\end{table}

==> tables/det_searching.tex <==
% \begin{table}
% % \footnotesize
% \centering
% % \begin{center}
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{c c || c c }
% \toprule
% % Searching & Top-1 & Reference & Top-1 \\
% % area size & Acc.  &  frame frequency & Acc.  \\
% \makecell{Searching\\area size} & \makecell{Top-1\\Acc.($\%$)} & \makecell{Reference\\anchor frequency} & \makecell{Top-1\\Acc.($\%$)} \\
% \midrule
% 1.25$\times$ & $52.4$  & 0  &  $49.7$ \\
% 1.5$\times$ & $52.7$  & 5 &  $52.8$ \\
% 2.0$\times$ & $52.5$ & 10   &  $52.3$ \\
% 2.5$\times$ & $52.1$ & 20  &  $50.2$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation studies on the searching area size and reference anchor frequency. The size of the searching area does not affect the overall performance of our method. The top-1 accuracy only varies 0.6\% while using different searching area sizes. This demonstrates the robustness of our MITFAS as the larger searching area contains more noises and outliers. %For reference anchor frequency, we perform the localization to obtain anchors to update the position of the searching area. We get the best accuracy when we use the anchors every 5 frames. The results also show that if we use the anchors more frequently, the overall accuracy will be higher. However, it is a trade-off between efficiency and performance, more anchors means more computational cost.
% }
% \vspace{-5pt}
% \label{tab:detsearching}
% % \end{center}
% \end{table}

\begin{table}
% \footnotesize
\centering
% \begin{center}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c c }
\toprule
% Searching & Top-1 & Reference & Top-1 \\
% area size & Acc.  &  frame frequency & Acc.  \\
Searching area size &  Top-1 Acc.($\%$)  \\
\midrule
1.25$\times$ reference size & $52.4$  \\
1.50$\times$ reference size & $52.7$   \\
2.00$\times$ reference size & $52.5$ \\
2.50$\times$ reference size & $52.1$  \\
\bottomrule
\end{tabular}
}
\caption{Ablation studies on the searching area size. The size of the searching area does not affect the overall performance of our method. The top-1 accuracy only varies 0.6\% while using different searching area sizes. This demonstrates the robustness of our MITFAS as the larger searching area contains more noises and outliers. %For reference anchor frequency, we perform the localization to obtain anchors to update the position of the searching area. We get the best accuracy when we use the anchors every 5 frames. The results also show that if we use the anchors more frequently, the overall accuracy will be higher. However, it is a trade-off between efficiency and performance, more anchors means more computational cost.
}
\vspace{-5pt}
\label{tab:detsearching}
% \end{center}
\end{table}
